Autonomous Drone Landing with Fiducial Markers and a Gimbal-Mounted Camera for Active Tracking

Precision landing is a remaining challenge in autonomous drone flight. Fiducial markers provide a computationally cheap way for a drone to locate a landing pad and autonomously execute precision landings. However, most work in this field depends on either rigidly-mounted or downward-facing cameras which restrict the drone's ability to detect the marker. We present a method of autonomous landing that uses a gimbal-mounted camera to quickly search for the landing pad by simply spinning in place while tilting the camera up and down, and to continually aim the camera at the landing pad during approach and landing. This method demonstrates successful search, tracking, and landing with 4 of 5 tested fiducial systems on a physical drone with no human intervention. Per fiducial system, we present the distributions of the distances from the drone to the center of the landing pad after each successful landing. We also show representative examples of flight trajectories, marker tracking performance, and control outputs for each channel during the landing. Finally, we discuss qualitative strengths and weaknesses underlying each system.

==> autogenerated/kruskal.tex <==
\begin{tabular}{rr}
\toprule
 $p_{\forall=}$ &     $H$ \\
\midrule
       0.006065 & 12.4235 \\
\bottomrule
\end{tabular}


==> autogenerated/overview.tex <==
\begin{tabular}{lrr}
\toprule
         System &  Successes &  Failures \\
\midrule
April Tag 48h12 &         20 &         3 \\
April Tag 24h10 &         20 &         5 \\
WhyCode Ellipse &         20 &         2 \\
   WhyCode Orig &         20 &         4 \\
  WhyCode Multi &          0 &        10 \\
\bottomrule
\end{tabular}


==> autogenerated/wilcoxon_pairwise.tex <==
\begin{tabular}{llrr}
\toprule
       System 1 &        System 2 &  $p_=$ & $p_\geq$ \\
\midrule
April Tag 48h12 & April Tag 24h10 &  0.014 &    0.007 \\
April Tag 48h12 & WhyCode Ellipse &  0.001 &    0.000 \\
April Tag 48h12 &    WhyCode Orig &  0.005 &    0.003 \\
April Tag 24h10 & April Tag 48h12 &  0.014 &    0.993 \\
April Tag 24h10 & WhyCode Ellipse &  0.701 &          \\
April Tag 24h10 &    WhyCode Orig &  1.000 &          \\
WhyCode Ellipse & April Tag 48h12 &  0.001 &    1.000 \\
WhyCode Ellipse & April Tag 24h10 &  0.701 &          \\
WhyCode Ellipse &    WhyCode Orig &  0.643 &          \\
   WhyCode Orig & April Tag 48h12 &  0.005 &    0.997 \\
   WhyCode Orig & April Tag 24h10 &  0.985 &          \\
   WhyCode Orig & WhyCode Ellipse &  0.643 &          \\
\bottomrule
\end{tabular}


==> sections/conclusion.tex <==
\label{section:conclusion}

We have shown that autonomous precision landing is possible with fiducial markers and a gimbal-mounted camera for active tracking.
Even with high processing latency,
4 of 5 tested systems have demonstrated success in the real world.
%While our platform does not have onboard processing hardware,
While our platform does not allow for on onboard companion board,
all essential image processing and control signal generation
is occurs in real time onboard a Raspberry Pi,
meaning that the entire system can be embedded onto a larger drone.
We have also demonstrated that
the gimbal-mounted camera setup allows the drone to search for the landing pad by simply
spinning in place and sweeping its gimbal up and down,
thereby safely and efficiently scanning a large area.


==> sections/future_work.tex <==
\label{section:future_work}

The next step is to re-conduct the experiments with the following changes:
embed the companion board into a larger drone to reduce the system's latency,
Use a gimbal that is able to point backwards to potentially improve WhyCode Multi's performance.
Extensions of this work should explore methods for filtering erroneous control signals
that result from orientation ambiguity,
or use an IMU on the drone's camera
to remove the problem of orientation ambiguity altogether.

